3D Textured Shape Recovery with Learned Geometric Priors

3D textured shape recovery from partial scans is crucial for many real-world applications. Existing approaches have demonstrated the efficacy of implicit function representation, but they suffer from partial inputs with severe occlusions and varying object types, which greatly hinders their application value in the real world. This technical report presents our approach to address these limitations by incorporating learned geometric priors. To this end, we generate a SMPL model from learned pose prediction and fuse it into the partial input to add prior knowledge of human bodies. We also propose a novel completeness-aware bounding box adaptation for handling different levels of scales and partialness of partial scans.

==> figures/2_post_processing.tex <==
\begin{figure}[ht]
  \centering
  % include first image
  \includegraphics[width=1\linewidth]{images/post_processing.jpg}  
  \caption{Diagram of shape fusion. Only the reconstruction results of the missing regions are preserved.}
  \label{fig:post_processing}
\end{figure}

==> figures/track1_score.tex <==
\begin{figure}[ht]
 \centering
  % include first image
  \includegraphics[width=0.95\linewidth]{images/track1_score.png}  
 

  \caption{Result list of track 1. Our team name is rayee. We rank 3rd in this track and have fairly little gap to the 2nd place. }
  \label{fig:track1score}
\end{figure}

==> figures/track2_score.tex <==
\begin{figure}[ht]
 \centering
  % include first image
  \includegraphics[width=0.95\linewidth]{images/track2_score.png}  
 
  \caption{Result list of track 2. We finally take the champion in this track. The quantitative validation score of shape and texture reaches a high level.}
  \label{fig:track2score}
\end{figure}
